The Mechanics of Nucleation and Growth and the Surface Tensions of Active Matter

Homogeneous nucleation, a textbook transition path for phase transitions, is typically understood on thermodynamic grounds through the prism of classical nucleation theory. However, recent studies have suggested the applicability of classical nucleation theory to systems far from equilibrium. In this Article, we formulate a purely mechanical perspective of homogeneous nucleation and growth, elucidating the criteria for the properties of a critical nucleus without appealing to equilibrium notions. Applying this theory to active fluids undergoing motility-induced phase separation, we find that nucleation proceeds in a qualitatively similar fashion to equilibrium systems, with concepts such as the Gibbs-Thomson effect and nucleation barriers remaining valid. We further demonstrate that the recovery of such concepts allows us to extend classical theories of nucleation rates and coarsening dynamics to active systems upon using the mechanically-derived definitions of the nucleation barrier and surface tensions. Three distinct surface tensions -- the mechanical, capillary, and Ostwald tensions -- play a central role in our theory. While these three surface tensions are identical in equilibrium, our work highlights the distinctive role of each tension in the stability of active interfaces and the nucleation and growth of motility-induced phases.

==> custom-commands.tex <==
\usepackage{multirow}

% ******** CUSTOMIZATIONS  ******** %
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

%******** FONT FORMATTING ********%
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
%new command
\newcommand{\xmark}{\ding{55}}%
\newcommand*\diff{\mathop{}\!\mathrm{d}}

%When editing
%\newcommand{\ed}[1]{{\color{blue}#1}}
\newcommand{\ed}[1]{{\color{black}#1}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

\makeatletter
\DeclareRobustCommand{\svdots}{%
  \hbox{ }\vbox{%
    \baselineskip 3\p@
    \lineskiplimit \z@
    \kern 1\p@
    \hbox{.}\hbox{.}\hbox{.}%
  }%
  \hbox{ }
}
\makeatother

\makeatletter
\def\overvect@#1#2#3{\vbox{\ialign{##\crcr
       \noalign{\kern-.7pt\nointerlineskip}#1#2\crcr
       \noalign{\kern1pt\nointerlineskip}$\m@th\hfil#2#3\hfil$\crcr}}}
\makeatother
\def\*#1{\mathbf{#1}}
%\newcommand{\todo}[1]{\textcolor{RedViolet}{[ToDo: #1]}}
\newcommand{\fvect}[1]{\overset{\rightarrow}{#1}}
\newcommand{\bvect}[1]{\overset{\leftarrow}{#1}}
\newcommand{\scp}{\mathcal{P}}
\newcommand{\bscp}{\partial \scp}

\DeclareMathOperator\erfc{erfc}
% increase line spacing in matrix environments
\makeatletter
\renewcommand*\env@matrix[1][\arraystretch]{%
  \edef\arraystretch{#1}%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols c}}
\makeatother

% better circled text
\newcommand*\circled[1]{
	\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=1pt] (char) {#1};
	}
}
%coloring in math mode
\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

%short arrow that can rotate
\makeatletter
\newcommand{\fixed@sra}{$\vrule height 2\fontdimen22\textfont2 width 0pt\shortrightarrow$}
\newcommand{\shortarrow}[1]{%
  \mathrel{\text{\rotatebox[origin=c]{\numexpr#1*45}{\fixed@sra}}}
}
\makeatother
\makeatletter
\newcommand{\blankarrow}{\textcolor{white}{\shortarrow{1}}}
\makeatother

%boxing characters
\makeatletter
\renewcommand{\boxed}[1]{\text{\fboxsep=.2em\fbox{\m@th$\displaystyle#1$}}}
\makeatother

%small fraction
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}
%\geometry{margin=1in}

%short to
\newcommand{\shortto}[1][3pt]{\mathrel{%
   \hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
   \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\def\doubleunderline#1{\underline{\underline{#1}}}

%TikZ code "illustrating" the new "brace"
\newcommand{\newbrace}[1][]{
\begin{tikzpicture}[baseline=-0.5ex]
\draw[#1] (0,0) -- (0.3,0.3);
\draw[#1] (0,0) -- (0.3,-0.3);
\end{tikzpicture}
}

% the optional argument allows you to select the type of arrow 
% you can also customize the "new brace"
\newenvironment{casesnew}[1][->]%
{\;\newbrace[#1]\;\begin{array}{@{}l@{}}}%
{\end{array}}

%Declaring some math operators
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\sech}{sech}
\allowdisplaybreaks

\renewcommand{\thefigure}{S.\arabic{figure}}
\renewcommand{\thetable}{S.\arabic{table}}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\DontPrintSemicolon
% Define pseudocode formatting
\renewcommand{\KwSty}[1]{\textnormal{\textcolor{blue!90!black}{\ttfamily\bfseries #1}}\unskip}
\renewcommand{\ArgSty}[1]{\textnormal{\ttfamily #1}\unskip}
\SetKwComment{Comment}{\color{green!50!black}// }{}
\renewcommand{\CommentSty}[1]{\textnormal{\ttfamily\color{green!50!black}#1}\unskip}
\newcommand{\assign}{\leftarrow}
\newcommand{\var}{\texttt}
\newcommand{\FuncCall}[2]{\texttt{\bfseries #1(#2)}}
\SetKwProg{Function}{function}{}{}
\renewcommand{\ProgSty}[1]{\texttt{\bfseries #1}}


%%%%%%%%%%%%%%%%%%%%%%% Wide tilde %%%%%%%%%%%%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{stackengine}
\usepackage{scalerel}
